Verifying Sierpi\'nski and Riesel Numbers in ACL2

A Sierpinski number is an odd positive integer, k, such that no positive integer of the form k * 2^n + 1 is prime. Similar to a Sierpinski number, a Riesel number is an odd positive integer, k, such that no positive integer of the form k * 2^n + 1 is prime. A cover for such a k is a finite list of positive integers such that each integer j of the appropriate form has a factor, d, in the cover, with 1 < d < j. Given a k and its cover, ACL2 is used to systematically verify that each integer of the given form has a non-trivial factor in the cover.

==> eptcsdata.tex <==
\providecommand{\firstpage}{20}
\providecommand{\publicationstatus}{Hardin and Schmaltz (Eds): ACL2 2011\\
EPTCS 70, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.70.2}{10.4204/EPTCS.70.2}}

